SHiP as a (post-)discovery machine: identifying the diphoton signals' origin

The upcoming SHiP experiment may probe interaction strengths of decaying feebly coupled particles several orders of magnitude below existing limits. In the event of a discovery, it may also reveal the nature of the new particle. This requires identifying its exact production mechanism, which SHiP does not observe directly. We explore whether this mechanism can be inferred from the kinematics of its visible decays. As a benchmark, we consider an axion-like particle (ALP) with a dominant diphoton decay, which may occur for couplings to the $U(1)_Y$ and $SU(2)_L$ gauge fields. For a known ALP mass, the observed energy and angular distributions depend on the relative magnitude and sign of the couplings and on the unknown lifetime, which we profile independently under each hypothesis. We first determine how the ALP energy and its longitudinal and transverse decay positions distinguish the interactions, assuming perfect reconstruction and accounting for production, propagation, decay, and geometric acceptance. We then include the detector response and reconstruct the diphoton decays using a full simulation of the SHiP electromagnetic calorimeter. Only $2$--$4$ reconstructed diphoton events are needed to distinguish the two pure $U(1)_{Y}$ and $SU(2)_{L}$ interactions for ALP masses between $0.2$ and $1~\mathrm{GeV}$. For coupling admixtures, the study assuming perfect reconstruction indicates requirements of several tens to $\mathcal{O}(10^2)$ events in favorable regions.

==> header.tex <==
\RequirePackage[colorlinks=true,
  urlcolor=blue,
  citecolor=blue,
  linkcolor=blue,
  linktocpage=true]{hyperref}

\usepackage{amsmath,amssymb,amsfonts}
\usepackage{graphicx}
\usepackage{booktabs}
\usepackage{tabularx}
\usepackage{array}
\usepackage{xcolor}
\usepackage{multirow}
\usepackage{enumitem}
\usepackage{placeins}
\usepackage{cleveref}
\usepackage{xspace}
\usepackage{siunitx}

\setlist[itemize]{leftmargin=1.4em,itemsep=0.15em,topsep=0.35em}

\newcommand{\diff}{\mathrm{d}}
\newcommand{\br}{\mathrm{Br}}
\newcommand{\gev}{\mathrm{GeV}}
\newcommand{\mev}{\mathrm{MeV}}
\newcommand{\tev}{\mathrm{TeV}}
\newcommand{\m}{\ensuremath{\mathrm{m}}\xspace}
\newcommand{\cm}{\ensuremath{\mathrm{cm}}\xspace}
\newcommand{\pot}{\mathrm{POT}}
\newcommand{\SUtwo}{\mathrm{SU}(2)_L}
\newcommand{\gagg}{g_{a\gamma\gamma}}
\newcommand{\rperp}{r_{\perp}}
\newcommand{\Nninety}{N_{90\%}}

\newcommand{\Malte}[1]{{\color{violet!80!black}\textbf{MALTE:} #1}}
\newcommand{\Matei}[1]{{\color{red!75!black}\textbf{MATEI:} #1}}
\newcommand{\EventCalc}[1]{{\color{blue!70!black}\textbf{EVENTCALC:} #1}}
\newcommand{\Authors}[1]{{\color{orange!60!black}\textbf{AUTHORS:} #1}}

\newcommand{\placeholderbox}[2]{%
  \begin{center}
  \setlength{\fboxsep}{8pt}%
  \fcolorbox{red!65!black}{red!3}{%
    \begin{minipage}{0.91\linewidth}
      \textbf{#1}\par\smallskip
      \small #2
    \end{minipage}}
  \end{center}%
}

\newcommand{\placeholderfigure}[2]{%
  \setlength{\fboxsep}{8pt}%
  \fcolorbox{blue!65!black}{blue!2}{%
    \begin{minipage}[c][0.22\textheight][c]{0.91\linewidth}
      \centering
      \textbf{FIGURE PLACEHOLDER: #1}\par\medskip
      \small #2
    \end{minipage}}%
}

\newcolumntype{Y}{>{\raggedright\arraybackslash}X}

\crefname{section}{Sec.}{Secs.}
\crefname{subsection}{Sec.}{Secs.}
\crefname{figure}{Fig.}{Figs.}
\crefname{table}{Table}{Tables}
\crefname{equation}{Eq.}{Eqs.}
\crefname{appendix}{Appendix}{Appendices}

\bibliographystyle{utphys}

